Perturbation-based Regret Analysis of Predictive Control in Linear Time Varying Systems

We study predictive control in a setting where the dynamics are time-varying and linear, and the costs are time-varying and well-conditioned. At each time step, the controller receives the exact predictions of costs, dynamics, and disturbances for the future $k$ time steps. We show that when the prediction window $k$ is sufficiently large, predictive control is input-to-state stable and achieves a dynamic regret of $O(\lambda^k T)$, where $\lambda < 1$ is a positive constant. This is the first dynamic regret bound on the predictive control of linear time-varying systems. Under more assumptions on the terminal costs, we also show that predictive control obtains the first competitive bound for the control of linear time-varying systems: $1 + O(\lambda^k)$. Our results are derived using a novel proof framework based on a perturbation bound that characterizes how a small change to the system parameters impacts the optimal trajectory.

==> Proofs/ISS_stability.tex <==
We will follow the standard Lyapunov function approach to show the input-to-state stability (ISS) of our MPC algorithm. We will use the following Lyapunov theorem for ISS, the proof of which can be found in \cite{jiang2001Lyapunov} as Lemma 3.5.

\begin{theorem}[Lyapunov theorem for ISS]\label{thm:Lyapunov-theorem-ISS}
Suppose we may design an \textit{ISS Lyapunov function} $V: \mathbb{N} \times \mathbb{R}^n \to \mathbb{R}_+$ for a time-varying system with dynamics $x_{t+1} = g_t(x_t, w_t)$, where there exists class-$K_{\infty}$ functions $\alpha_1, \alpha_2, \alpha_3$ and a class-$K$ function $\sigma$, such that the following inequalities hold for all $t \in \mathbb{N}$, $x \in \mathbb{R}^n$ and $w \in \mathbb{R}^n$:
\begin{gather*}
    \alpha_1(\norm{x}) \leq V(t, x) \leq \alpha_2(\norm{x}),\\
    V(t+1, g_t(x,w)) - V(t,x) \leq - \alpha_3(\norm{x}) + \sigma(\norm{w}).
\end{gather*}
Then the time-varying system is ISS. 
\end{theorem}

The above Lyapunov theorem is able to show that our MPC algorithm with replan window 1 is ISS, where the ISS Lypunov function is selected as the cost-to-go function.

\begin{theorem}[ISS of MPC with replan window 1]\label{thm:1-MPC-ISS-stability}
Suppose the online control system controlled by MPC satisfies the following additional constraints:

\begin{enumerate}
    \item there exists a class-$K_{\infty}$ function such that, at any time step $t+\tau$ ($1 \leq \tau \leq k$), 
    $$f_{t+\tau}(x_{t+\tau}) + c_{t+\tau}(u_{t+\tau-1}) \geq \alpha_{1} \left( \norm{(x_t, w_{t+1:t+k})} \right);$$
    
    \item there exists a class-$K_{\infty}$ function $\alpha_2$ such that
    $$F(x) \leq \alpha_2(\norm{x});$$
    
    \item there exists an auxiliary controller $\horizonvar: \mathbb{R}^n \to \mathbb{R}^m$ that is feasible;
    
    \item at any time step $t$, the terminal cost satisfies
    $$F \left( A_t x_t + B_t \horizonvar(x_t) + w_t \right) - F(x_t) \leq - \left( f_t(x_t) + c_t(\horizonvar(x_{t-1})) \right).$$
\end{enumerate}
Then the system is ISS with equilibrium $0$.
\end{theorem}

\begin{proof}[Proof of Theorem \ref{thm:1-MPC-ISS-stability}]
Let $J(t, x_t, v_{t:t+k-1})$ denote the total cost of the $k$-step trajectory generated by initial state $x_t$ and control sequence $v_{t:t+k-1}$, i.e.,
$$J(t, x_t, v_{t:t+k-1}) := \sum_{\tau=t+1}^{t+k} \left( f_{\tau}(x_{\tau}) + c_{\tau}(v_{\tau-1}) \right).$$
We proceed by showing that the total cost function of the $k$-step MPC controller
$$V(t, (x_t, w_{t+1:t+k})) := J(t, x_t, \tilde{\psi}_{t}^{k}(x_t, w_{t+1:t+k})_{v_{0:k-1}})$$
is an ISS Lyapunov function. Consider the following trajectories with initial state $(x_t, w_{t+1:t+k})$:
\begin{enumerate}
    \item the optimal control sequence starting from time $t$
    $$u^*_{t:t+k-1} = \left( u_{t}^*, \cdots, u_{t+k-1}^* \right) = \tilde{\psi}_{t}^{k}(x_t, w_{t+1:t+k})_{v_{0:k-1}};$$
    
    \item the shifted control sequence starting from time $(t+1)$
    $$u_{t+1:t+k} := \left( u_{t+1}^*, \cdots, u_{t+k-1}^*, \horizonvar \left( x^*_{t+k} \right) \right),$$
    where $x^*_{t+k} = \tilde{\psi}_{t}^{k}(x_t, w_{t+1:t+k})_{y_k}$ is the final state in the optimal trajectory;
    
    \item the auxiliary control sequence starting from time $(t+1)$: $\tilde{u}_{t+1:t+k} := \left( \tilde{u}_{t+1}, \cdots, \tilde{u}_{t+k} \right)$, along with the state sequence $\tilde{x} := \left( \tilde{x}_{t+1}, \cdots, \tilde{x}_{t+k} \right)$, generated by auxiliary controller $\horizonvar$:
    $$\tilde{x}_{t+\tau} := A\tilde{x}_{t+\tau-1} + B\tilde{u}_{t+\tau-1} + w_{t+\tau},\quad
      \tilde{u}_{t+\tau} := \horizonvar \left( \tilde{x}_{t+\tau} \right).$$
\end{enumerate}

The lower bound of $V(t, (x_t, w_{t+1:t+k}))$ is given by assumption (1) as
$$V(t, (x_t, w_{t+1:t+k})) \geq f_{t+1}(x_{t+1}) + c_{t+1}(u_t) \geq \alpha_{1} \left( \norm{(x_t, w_{t+1:t+k})} \right).$$

The upper bound of $V(t, (x_t, w_{t+1:t+k}))$ is shown via $J(t, x_t, \tilde{u}_{t:t+k-1})$. Assumption (4) gives
\begin{align*}
    F(\tilde{x}_{t+1}) - F(\tilde{x}_t) + \left( f_{t+1}(\tilde{x}_{t+1}) + c_{t+1} \left( \tilde{u}_t \right) \right) &\leq 0, \\
    F(\tilde{x}_{t+2}) - F(\tilde{x}_{t+1}) + \left( f_{t+2}(\tilde{x}_{t+2}) + c_{t+2} \left( \tilde{u}_{t+1} \right) \right) &\leq 0, \\
    \cdots\qquad& \\
    F(\tilde{x}_{t+k}) - F(\tilde{x}_{t+k-1}) + \left( f_{t+k}(\tilde{x}_{t+k}) + c_{t+k} \left( \tilde{u}_{t+k-1} \right) \right) &\leq 0,
\end{align*}
and the above $k$ inequalities add up to (after proper rearrangement of terms)
$$J(t, x_t, \tilde{u}_{t+1:t+k}) \leq F(x_t) \leq \alpha_2 \left( \norm{x_t} \right).$$
Now by the optimality of $u^*_{t:t+k-1}$ and assumption (2), we have
$$V(t, (x_t, w_{t+1:t+k})) = J(t, x_t, u^*_{t:t+k-1}) \leq J(t, x_t, \tilde{u}_{t:t+k-1}) \leq \alpha_2 \left( \norm{x_t} \right) \leq \alpha_2 \left( \norm{(x_t, w_{t+1:t+k})} \right).$$

The upper bound of the difference of Lyapunov function values in consecutive steps is given by
\begin{align*}
    &V(t+1, (x_{t+1}, w_{t+2:t+k+1})) - V(t, (x_t, w_{t+1:t+k})) \\
    {}={}& J \left( t+1, x_{t+1}, u^*_{k+1} \right) - J \left( t, x_t, u^*_t \right) \\
    {}\leq{}& J \left( t+1, x_{t+1}, u_{k+1} \right) - J \left( t, x_t, u^*_t \right) \\
    {}={}& -\left( f_{t+1}(x_{t+1}) + c_{t+1}(u^*_t) \right) + \left[ F(x_{t+k+1}) - F(x^*_{t+k}) + \left( f_{t+k+1}(x_{t+k+1}) + c_{t+k+1}(u_{t+k}) \right) \right]\\
    {}\leq{}& -\left( f_{t+1}(x_{t+1}) + c_{t+1}(u^*_t) \right) \\
    {}\leq{}& - \alpha_1 \left( \norm{(x_t, w_{t+1:t+k})} \right) + 0.
\end{align*}
Therefore, $V(t, (x_t, w_{t+1:t+k}))$ is indeed an ISS Lyapunov function, and the time-varying system is ISS with equilibrium $0$.
\end{proof}

==> Proofs/competitive_ratio.tex <==
To simplify the notation, we still omit the disturbance sequence $w_{t:t+k-1}$ in $\tilde{\psi}_t^k$ and $\psi_t^k$ throughout the proof. At each time step $t$, we will use $x_t/u_t$ to denote the state/input of $PC_{(k, h)}$ algorithm and use $x_t^*/ u_t^*$ to denote the state/input of the offline optimal. We define
\begin{align*}
    H_t &:= f_t(x_t), M_t := c_t(u_{t-1}),\\
    H_t^* &:= f_t(x_t^*), M_t^* := c_t(u_{t-1}^*).
\end{align*}
Let $\tilde{x}_{t + k} := \tilde{\psi}_{t}^k(x_t^*; F)_{y_k}, \bar{x}_{t+k} = \tilde{\psi}_{t}^k(x_t^*; 0)_{y_k}$.

If $t \leq T - k, t \equiv 0 (\text{mod }h)$, we have
\begin{subequations}\label{thm:MPC-CR-general:e0}
\begin{align}
    &\norm{x_{t+h} - x_{t+h}^*}^2\nonumber\\
    ={}& \norm{\tilde{\psi}_{t}^k(x_t; F)_{y_h} - \psi_{t}^k(x_t^*, x_{t+k}^*)_{y_h}}^2\nonumber\\
    \leq{}& \left(\norm{\tilde{\psi}_{t}^k(x_t; F)_{y_h} - \tilde{\psi}_{t}^k(x_t^*; F)_{y_h}} + \norm{\tilde{\psi}_{t}^k(x_t^*; F)_{y_h} - \psi_{t}^k(x_t^*, x_{t+k}^*)_{y_h}}\right)^2 \label{thm:MPC-CR-general:e0:s1}\\
    \leq{}& (1 + \epsilon) \norm{\tilde{\psi}_{t}^k(x_t; F)_{y_h} - \tilde{\psi}_{t}^k(x_t^*; F)_{y_h}}^2 + \left(1 + \frac{1}{\epsilon}\right) \norm{\tilde{\psi}_{t}^k(x_t^*; F)_{y_h} - \psi_{t}^k(x_t^*, x_{t+k}^*)_{y_h}}^2 \label{thm:MPC-CR-general:e0:s2}\\
    \leq{}& (1 + \epsilon) \norm{\tilde{\psi}_{t}^k(x_t; F)_{y_h} - \tilde{\psi}_{t}^k(x_t^*; F)_{y_h}}^2 + \left(1 + \frac{1}{\epsilon}\right) \norm{\psi_{t}^k(x_t^*, \tilde{x}_{t + k})_{y_h} - \psi_{t}^k(x_t^*, x_{t+k}^*)_{y_h}}^2 \label{thm:MPC-CR-general:e0:s3}\\
    \leq{}& (1 + \epsilon) C^2 \decayvar^{2h} \norm{x_t - x_t^*}^2 + C^2 \decayvar^{2(k - 1 - h)}\cdot \left(1 + \frac{1}{\epsilon}\right) \norm{x_{t+k}^* - \tilde{x}_{t +k}}^2 \label{thm:MPC-CR-general:e0:s4}\\
    \leq{}& \frac{1}{1 + \epsilon}\norm{x_t - x_t^*}^2 + C^2 \decayvar^{2(k - 1 - h)}\cdot \left(1 + \frac{1}{\epsilon}\right) \norm{x_{t+k}^* - \tilde{x}_{t +k}}^2, \label{thm:MPC-CR-general:e0:s5} 
\end{align}
\end{subequations}
where we use the triangle inequality in \eqref{thm:MPC-CR-general:e0:s1}, the AM-GM inequality in \eqref{thm:MPC-CR-general:e0:s2}, the definition of $\tilde{x}_{t+k}$ in \eqref{thm:MPC-CR-general:e0:s3}, Theorem \ref{thm:LTV-sensitivity} in \eqref{thm:MPC-CR-general:e0:s4}, and the assumption on $h$ in \eqref{thm:MPC-CR-general:e0:s5}.

%To obtain an upper bound of $\norm{x_{t+k}^* - \tilde{x}_{t +k}}^2$, we define $\bar{x}_{t+k}$ as the value of $\tilde{x}_{t+k}$ when the terminal cost $F(\cdot)$ is set to be zero. 
Since the objective function is $m_f$-strongly convex in variables $x_{t+1:t+k}$, we see that
\begin{equation}\label{thm:MPC-CR-general:e0-1}
    \norm{x_{t+k}^* - \bar{x}_{t +k}}^2 \leq \frac{2}{m_f}\sum_{\tau = 1}^{k}(H_{t + \tau}^* + M_{t + \tau}^*).
\end{equation}
Since $f_{t+k}$ is $m_f$-strongly convex, we also see that $\norm{x_{t+k}^*}^2 \leq \frac{2}{m_f}H_{t+k}^*$. Recall that the terminal cost $F(x_{t+k}) = \alpha(\norm{x_{t+k}})$, where $\alpha$ is a K-function. By the definition of $\tilde{\psi}$, we see that $\norm{\tilde{x}_{t+k}} \leq \norm{\bar{x}_{t+k}}$. Therefore, we obtain that
\begin{subequations}\label{thm:MPC-CR-general:e1}
\begin{align}
    \norm{x_{t+k}^* - \tilde{x}_{t+k}}^2 &\leq 2\norm{\tilde{x}_{t+k}}^2 + 2\norm{x_{t+k}^*}^2\label{thm:MPC-CR-general:e1:s1}\\
    &\leq 2\norm{\bar{x}_{t+k}}^2 + 2\norm{x_{t+k}^*}^2\label{thm:MPC-CR-general:e1:s2}\\
    &\leq 4\norm{\bar{x}_{t+k} - x_{t+k}^*}^2 + 6\norm{x_{t+k}^*}^2\label{thm:MPC-CR-general:e1:s3}\\
    &\leq \frac{8}{m_f}\sum_{\tau = 1}^{k}(H_{t + \tau}^* + M_{t + \tau}^*) + \frac{12}{m_f}H_{t+k}^*\label{thm:MPC-CR-general:e1:s4}\\
    &\leq \frac{20}{m_f}\sum_{\tau = 1}^{k}(H_{t + \tau}^* + M_{t + \tau}^*),\nonumber
\end{align}
\end{subequations}
where we use Cauchy-Schwarz inequality in \eqref{thm:MPC-CR-general:e1:s1} and \eqref{thm:MPC-CR-general:e1:s3}, $\norm{\tilde{x}_{t+k}} \leq \norm{\bar{x}_{t+k}}$ in \eqref{thm:MPC-CR-general:e1:s2}, and \eqref{thm:MPC-CR-general:e0-1} in \eqref{thm:MPC-CR-general:e1:s4}.

Suppose $T = n_0\cdot h + m_0$, where $n_0 \in \mathbb{Z}_+$ and $k - h + 1 \leq m_0 \leq k$. By summing up inequality (\ref{thm:MPC-CR-general:e0}) for $t = 0, h, 2h, \ldots, (n - 1)h$, we obtain that
\begin{align}\label{equ:critical_point_seq_2}
    \sum_{i = 1}^{n_0} \norm{x_{i h} - x_{i h}^*}^2 &\leq C^2 \decayvar^{2(k - 1 - h)} \cdot \frac{(1 + \epsilon)^2}{\epsilon^2} \cdot \sum_{i = 1}^{n_0 - 1} \norm{x_{i h + k}^* - \tilde{x}_{i h + k}}^2\nonumber\\
    &\leq C^2 \decayvar^{2(k - 1 - h)} \cdot \frac{(1 + \epsilon)^2}{\epsilon^2} \cdot \frac{20}{m_f} \cdot cost(OPT),
\end{align}
where we use \eqref{thm:MPC-CR-general:e1} in the last inequality.

\yiheng{I think \eqref{equ:critical_point_seq_2} is wrong. The correct version should be
\begin{align*}
    \sum_{i = 1}^{n_0} \norm{x_{i h} - x_{i h}^*}^2 &\leq C^2 \decayvar^{2(k - 1 - h)} \cdot \frac{(1 + \epsilon)^2}{\epsilon^2} \cdot \sum_{i = 1}^{n_0 - 1} \norm{x_{i h + k}^* - \tilde{x}_{i h + k}}^2\nonumber\\
    &\leq C^2 \decayvar^{2(k - 1 - h)} \cdot \frac{(1 + \epsilon)^2}{\epsilon^2} \cdot \frac{20}{m_f} \cdot \frac{k}{h} \cdot cost(OPT).
\end{align*}
}

Therefore, we can show that, for all $\eta > 0$:
\begin{subequations}\label{equ:sliding_window_general_competitive_e1}
\begin{align}
    &cost(PC_{(k, h)}) - (1 + \eta) cost(OPT)\nonumber\\
    ={}& \left(\sum_{i = 0}^{n_0 - 1} \iota_{i h}^h(x_{i h}, x_{(i + 1) h}) + \iota_{n_0 h}^{m_0}(x_{n_0 h}, x_T)\right) - (1 + \eta)\left(\sum_{i = 0}^{n_0 - 1} \iota_{i h}^h(x_{i h}^*, x_{(i + 1) h}^*) + \iota_{n_0 h}^{m_0}(x_{n_0 h}^*, x_T^*)\right)\nonumber\\
    ={}& \sum_{i = 0}^{n_0 - 1} \left(\iota_{i h}^h(x_{i h}, x_{(i + 1) h}) - (1 + \eta)\iota_{i h}^h(x_{i h}^*, x_{(i + 1) h}^*)\right) + \left(\iota_{n_0 h}^{m_0}(x_{n h}, x_T) - (1 + \eta)\iota_{n_0 h}^{m_0}(x_{n h}^*, x_T^*)\right)\nonumber\\
    \leq{}& \sum_{i = 0}^{n_0 - 1} \left(\iota_{i h}^h(x_{i h}, x_{(i + 1) h}) - (1 + \eta)\iota_{i h}^h(x_{i h}^*, x_{(i + 1) h}^*)\right) + \left(\iota_{n_0 h}^{m_0}(x_{n h}, x_T^*) - (1 + \eta)\iota_{n_0 h}^{m_0}(x_{n h}^*, x_T^*)\right)\label{equ:sliding_window_general_competitive_e1:s1}\\
    \leq{}& \left(1 + \frac{1}{\eta}\right)\cdot \frac{L_0+\ell_f}{2} \sum_{i = 0}^{n_0 - 1} \left(\norm{x_{i h} - x_{i h}^*}^2 + \norm{x_{(i + 1) h} - x_{(i + 1) h}^*}^2\right) + \left(1 + \frac{1}{\eta}\right)\cdot \frac{L_0+\ell_f}{2} \norm{x_{n_0 h} - x_{n_0 h}^*}^2\label{equ:sliding_window_general_competitive_e1:s2}\\
    ={}& \left(1 + \frac{1}{\eta}\right)\cdot (L_0 + \ell_f) \sum_{i = 1}^{n_0} \norm{x_{i h} - x_{i h}^*}^2\nonumber\\
    \leq{}& \left(1 + \frac{1}{\eta}\right)\cdot (L_0 + \ell_f) \cdot C^2 \decayvar^{2(k - 1 - h)} \cdot \frac{20(1 + \epsilon)^2}{m_f \epsilon^2} \cdot cost(OPT),\label{equ:sliding_window_general_competitive_e1:s3}
\end{align}
\end{subequations}
where we use the fact that the PC algorithm (with replan window $h$) plans optimally after time step $n h$ in \eqref{equ:sliding_window_general_competitive_e1:s1}; we also use Corollary \ref{coro:smooth-cost} in \eqref{equ:sliding_window_general_competitive_e1:s2}, and \eqref{equ:critical_point_seq_2} in \eqref{equ:sliding_window_general_competitive_e1:s3}.

By setting $\eta \sim \epsilon^{-1} \left(\frac{L_0 + \ell_f}{m_f}\right)^{\frac{1}{2}} \cdot C \decayvar^{k - 1 - h}$, we see that the competitive ratio of the $PC_{(k, h)}$ algorithm (with replan window $h$) is in the order of
\[1 + O\left(\epsilon^{-1}\left(\frac{L_0 + \ell_f}{m_f}\right)^{\frac{1}{2}} \cdot C \decayvar^{k - 1 - h}\right).\]



==> Proofs/mat_inverse.tex <==
% This is not used.
\begin{comment}
    We first show this lemma holds for the special case where $D_i = 0, i = 1, \ldots, n$. After giving the proof for this special case, we will show that the general case where $D_i \succeq 0$ can be reduced to this special case.
    
    For $i \not = j$, write $\abs{i - j} = nm/2 + k$ for $k = 1, \ldots, m/2$. Following the same approach as the proof of Proposition 2.2 in \cite{demko1984decay}, we see that there exists $p_n \in \pi_n$ such that
    \[\norm{A^{-1} - p_n(A)}_2 \leq C_0 \lambda^{\abs{i - j}}.\]
    Since $p_n(A)$ satisfies that $\left(p_n(A)\right)_{i, j} = 0$, we further obtain that
    \[\norm{\left(A^{-1}\right)_{i,j}}_2 \leq \norm{\left(A^{-1} - p_n(A)\right)_{i,j}}_2 \leq \norm{A^{-1} - p_n(A)}_2 \leq C_0 \lambda^{\abs{i - j}},\]
    where we used the fact that the induced 2-norm of a submatrix must be less than or equal to the 2-norm of the original matrix.
        
    For $i = j$, notice that $\norm{\left(A^{-1}\right)_{i, j}}_2 \leq \norm{A^{-1}}$. This finishes the proof for the special case.
    
    Now we show the general case by reducing it to the special case we have shown.
    
    Define matrix $M := (a I + D) \in \mathbb{S}^{nd}$. Define matrix $H \in \mathbb{S}^{nd}$ such that
    \[H = M^{-\frac{1}{2}} (A + D) M^{-\frac{1}{2}}.\]
    We first show that $\frac{b}{a}\cdot I \succeq H \succeq I$. For any $x \in \mathbb{R}^{nd}$, we see that
    \begin{align*}
        x^\intercal H x &= x^\intercal M^{-\frac{1}{2}}A M^{-\frac{1}{2}}x + x^\intercal M^{-\frac{1}{2}}D M^{-\frac{1}{2}}x\\
        &\geq x^\intercal M^{-\frac{1}{2}} aI M^{-\frac{1}{2}}x + x^\intercal M^{-\frac{1}{2}}D M^{-\frac{1}{2}}x\\
        &= x^\intercal M^{-\frac{1}{2}} (aI + D) M^{-\frac{1}{2}}x\\
        &= \norm{x}_2^2.
    \end{align*}
    For the other direction, we also have that
    \begin{align*}
        x^\intercal H x &= x^\intercal M^{-\frac{1}{2}}A M^{-\frac{1}{2}}x + x^\intercal M^{-\frac{1}{2}}D M^{-\frac{1}{2}}x\\
        &\leq x^\intercal M^{-\frac{1}{2}} bI M^{-\frac{1}{2}}x + x^\intercal M^{-\frac{1}{2}}D M^{-\frac{1}{2}}x\\
        &= x^\intercal M^{-\frac{1}{2}} (aI + D) M^{-\frac{1}{2}}x + (b - a) x^\intercal M^{-1} x\\
        &\leq \norm{x}_2^2 + \frac{b - a}{a} \cdot \norm{x}_2^2\\
        &= \frac{b}{a}\cdot \norm{x}_2^2.
    \end{align*}
    Thus $\frac{b}{a}\cdot I \succeq H \succeq I$. Since $H$ is $m$-banded, we can apply the special case result ($D_i = 0, i = 1, \ldots, n$) to obtain that
    \[\norm{(H^{-1})_{i,j}}_2 \leq C' \lambda^{\abs{i - j}},\]
    where $C' = \max\{1, \left(1 + \sqrt{\horizonvar(A)}\right)^2/(2 \horizonvar(A))\}$. Using this inequality, we further obtain that
    \begin{align*}
        \norm{((A + D)^{-1})_{i,j}}_2 &= \norm{\left(M^{-\frac{1}{2}} H^{-1} M^{-\frac{1}{2}}\right)_{i,j}}_2\\
        &\leq \norm{(aI + D_i)^{-\frac{1}{2}}}_2 \cdot \norm{(H^{-1})_{i,j}}_2 \cdot \norm{(aI + D_j)^{-\frac{1}{2}}}_2\\
        &\leq \frac{1}{a}\norm{(H^{-1})_{i,j}}_2\\
        &\leq C \lambda^{\abs{i - j}}.
    \end{align*}
\end{comment}

==> old_competitive.tex <==


We now focus on bounding the competitive ratio of predictive control.  Here, we study a modification of the predictive control algorithm we have considered to this point.  In particular, we introduce a replan window $h$, as defined in Algorithm \ref{alg:pc-replan}  which we denote as $PC_{(k, h)}$.  This style of algorithm has been considered previously in the SOCO literature, where it has been shown to obtain a constant competitive ratio in some settings where MPC does not \cite{chen2016using}.

Our analysis approach highlights why this modification is beneficial for competitive ratio. Specifically, we obtain the competitive ratio bound by applying a potential method building on~\cite{bansal2019potential}. We define the potential function as the squared distance between the algorithm's trajectory and the offline optimal trajectory, i.e.,
$\phi_t(x_t, x_t^*) = \norm{x_t - x_t^*}^2,$
which is standard in the literature \cite{goel2019beyond, goel2018smoothed,shi2020online}. We study how this potential function changes over time. Intuitively, we need to upper bound the increment of this potential function by the offline optimal cost to obtain a competitive ratio result. To achieve this, the algorithm needs to ``move closer'' to the offline optimal trajectory rather than ``moving further away'' from it. Recall that Theorem \ref{thm:LTV-sensitivity} gives that
\begin{equation}\label{equ:distance-change}
    \norm{\psi_t^k(x_t, w_{t:t+k-1}; F)_{y_h} - \psi_t^k(x_t^*, w_{t:t+k-1}; F)_{y_h}} \leq C \decayvar^h\norm{x_t - x_t^*}.
\end{equation}
When the algorithm commits the first predictive state ($h = 1$), the left hand side of \eqref{equ:distance-change} might be larger than $\norm{x_t - x_t^*}$ when $C\decayvar > 1$. Thus, the algorithm must ``wait'' until the right hand side of \eqref{equ:distance-change} becomes smaller than $\norm{x_t - x_t^*}$. This is accomplished in Algorithm \ref{alg:pc-replan} via the replan window $h$.

\begin{algorithm}[t]
\caption{Predictive Control with Replan Window $h$ ($PC_{(k, h)}$)}\label{alg:pc-replan}
\begin{algorithmic}[1]
\State Suppose $T = n_0 h + m_0$, where integers $n_0 \geq 0, k - h + 1 \leq m_0 \leq k$.
\For{$t = 0, h, \ldots, n_0 (h - 1)$}
    \State Observe current state $x_t$ and receive predictions $\vartheta_{t:t+k-1}$.
    \State Solve and commit control actions $u_{t:t+h-1} := \tilde{\psi}_t^k(x_t, w_{t:t+k-1}; F)_{v_{0:h-1}}$.
\EndFor
\State At time step $t = n_0 h$, observe current state $x_t$ and receive predictions $\vartheta_{t:T-1}$.
\State Solve and commit control actions $u_{t:T-1} := \tilde{\psi}_t^{m_0}(x_t, w_{t:T-1}; 0)_{v_{0:m_0-1}}$.
\end{algorithmic}
\end{algorithm}

Our main result for this section is the following competitive ratio bound for $PC_{(k, h)}$.

\begin{theorem}\label{thm:MPC-CR-general}
Let $\decayvar, C, L_0$ be the decay rate and constants defined in Theorem \ref{thm:LTV-sensitivity}. In Algorithm \ref{alg:pc-replan}, if the replan window $h$ satisfies
$h \geq \max\{\log{((1 + \varepsilon) C)}/\log{(1/\decayvar)}, d\}$ for some positive constant $\varepsilon$, and the prediction window $k$ satisfies $k \geq h + d$, then it has competitive ratio 
\[1 + O\left(\varepsilon^{-1}\left(\frac{L_0 + \ell_f}{m_f}\right)^{1/2} \cdot C \decayvar^{k - 1 - h}\right),\]
where the notation only hides a small numerical constant.
\end{theorem}

Note that when the constant $\varepsilon$ and the replan window $h$ are fixed, the competitive ratio is on the order of $1 + O(\rho^k)$ as the length of prediction $k$ tends to infinity. One potential line of future work is to understand if the replan window is necessary. It may be possible to either strengthen the constants given in Theorem \ref{thm:LTV-sensitivity} or improve our proof approach so as to eliminate the requirement on $h$.

%%\yiheng{Corollary for special case. Simplify the theorem's statement.}











\begin{comment}
\begin{lemma}\label{lemma:ISS-replan}
Under the same assumption as Theorem \ref{thm:MPC-CR-general}, the MPC algorithm with replan window $h$ is input-to-state stable.
\end{lemma}
\begin{proof}[Proof of Lemma \ref{lemma:ISS-replan}]
To simplify the notation, define $w_{sup} = \sup_{t\geq 0}\norm{w_t}$. By Corollary \ref{coro:opt-stable}, we see that for any non-negative integer $q$,
\[\norm{x_{(q + 1) h}} = \norm{\tilde{\phi}_t^k(x_{qh}, w_{qh:(q+1)h-1})_{y_h}} \leq C_1 \decayvar_1^h \norm{x_{qh}} + \frac{2 C_1}{1 - \decayvar_1} w_{sup} \leq \frac{1}{1 + \epsilon}\norm{x_{qh}} + \frac{2 C_1}{1 - \decayvar_1} w_{sup}.\]
Using the above inequality, we can show by induction that for any non-negative integer $q$,
\[\norm{x_{qh}} \leq \norm{x_0} + \frac{2(1 + \epsilon)C_1}{\epsilon (1 - \decayvar_1)}w_{sup}.\]
By Corollary \ref{coro:opt-stable}, we see that for any integer $1 \leq r \leq h-1$, we have
\begin{align*}
    \norm{x_{qh + r}} &= \norm{\tilde{\phi}_t^k(x_{qh}, w_{qh:(q+1)h-1})_{y_r}}\\
    &\leq C_1 \decayvar_1^r \norm{x_{qh}} + \frac{2 C_1}{1 - \decayvar_1} w_{sup}\\
    &\leq C_1 \norm{x_0} + \frac{2 C_1 ((1 + \epsilon)C_1 + \epsilon)}{(1 - \decayvar_1)\epsilon} w_{sup}.
\end{align*}
\end{proof}
\end{comment}
